Neural Spectral Decomposition for Dataset Distillation

In this paper, we propose Neural Spectrum Decomposition, a generic decomposition framework for dataset distillation. Unlike previous methods, we consider the entire dataset as a high-dimensional observation that is low-rank across all dimensions. We aim to discover the low-rank representation of the entire dataset and perform distillation efficiently. Toward this end, we learn a set of spectrum tensors and transformation matrices, which, through simple matrix multiplication, reconstruct the data distribution. Specifically, a spectrum tensor can be mapped back to the image space by a transformation matrix, and efficient information sharing during the distillation learning process is achieved through pairwise combinations of different spectrum vectors and transformation matrices. Furthermore, we integrate a trajectory matching optimization method guided by a real distribution. Our experimental results demonstrate that our approach achieves state-of-the-art performance on benchmarks, including CIFAR10, CIFAR100, Tiny Imagenet, and ImageNet Subset. Our code are available at \url{https://github.com/slyang2021/NSD}.

==> tables/del.tex <==
\begin{table*}
\centering
\scriptsize

\begin{minipage}{.56 \linewidth}
\centering
\setlength{\tabcolsep}{1.2mm}
\begin{tabular}{c|c|c|c|c}
        \toprule
         Group-SA & SA -D  &  CA -D  &params &mAP\\
         \midrule
         & &  & 47.6M&72.50\\
         % \hline
         \checkmark & & &47.6M&73.63(\textbf{$\uparrow$ 1.13}) \\
         \checkmark & \checkmark &  &49.2M&76.01(\textbf{$\uparrow$ 2.38})\\
         \checkmark &  \checkmark&  \checkmark&50.6M&76.83(\textbf{$\uparrow$ 0.82})\\
         \bottomrule
        \end{tabular}
\end{minipage}
\begin{minipage}{.40 \linewidth}
\caption{Ablation Study on the design of points detection decoder. SA means Self-Attention and CA means Cross-Attention. -D means decouple parameters for ${Q}_{bp}$ and ${Q}_{cp}$'s processing.}
\label{tab:DECODER}
\end{minipage}
\end{table*}

==> tables/feat_sim.tex <==
\begin{figure}[!ht]
\centering
\tiny
\vspace{-5mm}
\includegraphics[width=0.9\linewidth]{figs/rebuttal_sim.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\vspace{-2mm}
\caption{Cosine similarity of (a)synthetic dataset, (b)real dataset on CIFAR10}

% $\tau^*$ is the expert training trajectory intercepted in the initial training period using full dataset $D_{real}$, where each node $\vec{\theta}^*_t$ represents the trained weights of an epoch. The weight subspace $\mathbb{S}_{\tau^*}$ is spanned by $\{\vec{\theta}^*_t\}^T_0$. $\vec{G}$ is the parameter gradient vector generated when training the network with the synthetic dataset $D_{syn}$, and the subspace projection loss $l_{proj}$ is obtained by making a vector difference between $\vec{G}$ and its projection $\vec{G}_{\mathbb{S}_{\tau^*}}$ in $\mathbb{S}_{\tau^*}$.
\vspace{-0.25in}
\label{feat_sim}
\end{figure}

==> tables/rebuttal.tex <==
% \begin{center}
\begin{minipage}{\linewidth}
        \vspace{-0.2cm}
        \centering
        \begin{minipage}[t]{0.45\linewidth}
            % \captionsetup[table]{font={\tiny}}
            \begin{table}[H]
                \setlength{\abovecaptionskip}{-0cm}
                \setlength{\belowcaptionskip}{-0cm}
                \captionsetup{font=scriptsize}
                \caption{Different dataset.}
                \centering
                \resizebox{\linewidth}{!}{
                \begin{NiceTabular}{c|cc}
                    \toprule
                    & SVHN & CIFAR10 \\
                    \midrule
                    Ori IDC & 68.1\tiny$\pm$0.1 & 50.0\tiny$\pm$0.4\\
                    ESP IDC & \textbf{69.3\tiny$\pm$0.2} & \textbf{50.4\tiny$\pm$0.2}\\
                    \bottomrule
                \end{NiceTabular}
                }
                \label{tab3}
            \end{table}
        \end{minipage}
        % 中间不能有空格，否则不会并排显示
        \begin{minipage}[t]{0.45\linewidth}
            \begin{table}[H]
                \setlength{\abovecaptionskip}{-0cm}
                \setlength{\belowcaptionskip}{-0cm}
                \captionsetup{font=scriptsize}
                \caption{Cross architecture.}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{NiceTabular}{c|cc}
                    \toprule
                      & ResNet & DenseNet \\
                    \midrule
                    Ori IDC & 41.9\tiny$\pm$0.6 & 39.8\tiny$\pm$1.2\\
                    ESP IDC & \textbf{42.6\tiny$\pm$0.3} & \textbf{40.7\tiny$\pm$0.7}\\
                    \bottomrule
                    \end{NiceTabular}
                    }
                \label{tab3}
            \end{table}
        \end{minipage}
        % \begin{minipage}[t]{0.32\linewidth}
        %     \begin{table}[H]
        %         \setlength{\abovecaptionskip}{0cm}
        %         \setlength{\belowcaptionskip}{-0.2cm}
        %         \renewcommand\arraystretch{1.2}
        %         \captionsetup{font={tiny}}
        %         \caption{Backprop Ablation.}
        %         \centering
        %         \resizebox{\linewidth}{!}{
        %         \begin{NiceTabular}{c|ccc}
        %             \toprule
        %              N & 1 & 2 & 5 \\
        %             \midrule
        %             Ours & 63.0\tiny$\pm$0.4  & 63.0\tiny$\pm$0.3 & 62.3\tiny$\pm$0.3 \\
        %             N-back & 63.0\tiny$\pm$0.4 & 63.2\tiny$\pm$0.3 & 62.8\tiny$\pm$0.3 \\
                    
                    
        %             \bottomrule
        %         \end{NiceTabular}}
        %         \label{tab3}
        %     \end{table}
        % \end{minipage}
\end{minipage}
% \end{center}

% \begin{minipage}{0.9\linewidth}
%         \begin{minipage}[t]{0.45\linewidth}
%             \begin{table}[H]
%                 \centering
%                 \fontsize{9}{11}\selectfont
%                 \begin{tabular}{c|c|c|c}
%                     \toprule 
%                     $i$ & 0 & 1 & 2 \\ \midrule
%                     顶点 & V1 & V2 & V3 \\ \midrule
%                     $visited[i]$ & \textbf{\textit{1}} & 0 & 0 \\ \midrule
%                     $dist[i]$ & INF & \textbf{\textit{102}} & \textbf{\textit{99}} \\ \midrule
%                     $path[i]$ & $-1$ & \textbf{\textit{0}} & \textbf{\textit{0}} \\ \bottomrule
%                 \end{tabular}
%                 \caption{初始状态\label{初始状态}}
%                 \vspace{3pt}
%             \end{table}
%         \end{minipage}
%         % 中间不能有空格，否则不会并排显示
%         \begin{minipage}[t]{0.45\linewidth}
%             \begin{table}[H]
%                 \centering
%                 \fontsize{9}{11}\selectfont
%                 \begin{tabular}{c|c|c|c}
%                     \toprule 
%                     $i$ & 0 & 1 & 2 \\ \midrule
%                     顶点 & V1 & V2 & V3 \\ \midrule
%                     $visited[i]$ & 1 & 0 & \textbf{\textit{1}} \\ \midrule
%                     $dist[i]$ & INF & 102 & 99 \\ \midrule
%                     $path[i]$ & $-1$ & $0$ & $0$ \\ \bottomrule
            
%                 \end{tabular}
%                 \caption{选取顶点V3\label{选取顶点V3}}
%                 \vspace{3pt}
%             \end{table}
%         \end{minipage}
%     \end{minipage}

==> tables/rebuttal_ablation_t2.tex <==
\begin{table}[ht!]
\vspace{-0.15in}
\centering
\small
\setlength{\tabcolsep}{2.5mm}{
  \begin{tabular}{c|cccc}
  % & \multicolumn{4}{c}{\textbf{*** }} \\
   \toprule
   % \vspace{-0.15in}
% &\multicolumn{4}{c}{Evaluation Model}\\
   ($t_1$, $t_2$) & (48, 1) & (16, 3) & (10, 5) & (7, 7) \\
   \midrule
ours & 52.3$\pm$0.4 & \textbf{68.5$\pm$0.8} & 61.5$\pm$0.6 & 60.5$\pm$0.8\\
% 10&0.2& 65.3$\pm$0.7 & -\\

\bottomrule
     \end{tabular}}
     \vspace{-3mm}
     % \vspace{1em}
%   \caption{
% Comparison of test results for fixed $t_3$ and $t_4$ using different $t_2$ with (CIFAR10, IPC=1).}
\caption{Fixed $t_3$ and $t_4$ using different $t_2$ (CIFAR10, IPC=1).}
  \label{tab:t2}
  \vspace{-0.1in}
\end{table}

% 在CIFAR10数据集上IPC=1的情况下，固定t3和t4采用不同t2的测试结果对比

==> tables/rebuttal_ablation_t34.tex <==
% \begin{table}[ht!]
% \vspace{0.1in}
% \centering
% \small
% \setlength{\tabcolsep}{2.5mm}{
%   \begin{tabular}{c|cccc}
%   % & \multicolumn{4}{c}{\textbf{*** }} \\
%    \toprule
%    % \vspace{-0.15in}
% % &\multicolumn{4}{c}{Evaluation Model}\\
%    $t_3$$\backslash$$t_4$& 8 & 16 & 32 & 64\\
%    \midrule
% 8 &  57.5$\pm$0.3 & 58.1$\pm$0.7 & 59.6$\pm$0.2 & 56.2$\pm$0.3\\
% 16 &  59.4$\pm$0.4 & \textbf{68.5$\pm$0.8} & 61.2$\pm$0.6 & 40.1$\pm$0.5\\
% 32 &  60.4$\pm$0.7 & 61.5$\pm$0.3 & 57.9$\pm$0.4 & 53.7$\pm$0.5\\
% 64 &  58.1$\pm$0.7 & 42.4$\pm$0.9 & 53.9$\pm$0.5 & 36.1$\pm$0.6\\

% \bottomrule
%      \end{tabular}}
%      \vspace{-2mm}
%      % \vspace{1em}
%   \caption{
% Comparison of test results using different $t_3$ and $t_4$ for fixed $t_2$ with (CIFAR10, IPC=1).}
%   \label{tab:t34}
%   \vspace{-0.1in}
% \end{table}

\begin{table}[ht!]
\vspace{-0.2in}
\centering
\small
\setlength{\tabcolsep}{2.5mm}{
  \begin{tabular}{c|ccc}
  % & \multicolumn{4}{c}{\textbf{*** }} \\
   \toprule
   % \vspace{-0.15in}
% &\multicolumn{4}{c}{Evaluation Model}\\
   $t_3$$\backslash$$t_4$& 8 & 16 & 32\\
   \midrule
8 &  57.5$\pm$0.3 & 58.1$\pm$0.7 & 59.6$\pm$0.2\\
16 &  59.4$\pm$0.4 & \textbf{68.5$\pm$0.8} & 61.2$\pm$0.6\\
32 &  60.4$\pm$0.7 & 61.5$\pm$0.3 & 57.9$\pm$0.4\\

\bottomrule
     \end{tabular}}
     \vspace{-3mm}
     % \vspace{1em}
%   \caption{
% Comparison of test results using different $t_3$ and $t_4$ for fixed $t_2$ with (CIFAR10, IPC=1).}
\caption{Fixed $t_2$ using different $t_3$ and $t_4$ (CIFAR10, IPC=1).}
  \label{tab:t34}
  \vspace{-0.2in}
\end{table}
%固定t2使用不同t3和t4

==> tables/rebuttal_ftd.tex <==
% \begin{table}[ht!]
% \vspace{0.1in}
% \centering
% \small
% \setlength{\tabcolsep}{2.5mm}{
%   \begin{tabular}{c|cccc}
%   % & \multicolumn{4}{c}{\textbf{*** }} \\
%    \toprule
%    % \vspace{-0.15in}
% &\multicolumn{3}{c}{CIFAR10}\\
%    IPC & 1 & 10 & 50\\
%    Ratio\%& 0.02 & 0.2 & 1\\
%    \midrule
% FTD& 46.8$\pm$0.3 & 66.6$\pm$0.3 & 73.8$\pm$0.2 \\
% w.ours& 68.7$\pm$0.4 & 73.9$\pm$0.6 & -  \\

% \bottomrule
%      \end{tabular}}
%      \vspace{-2mm}
%      % \vspace{1em}
%   \caption{
% Test accuracy using FTD as benchmark method on CIFAR10.}
%   \label{tab:ftd}
%   \vspace{-0.1in}
% \end{table}

\begin{table}[ht!]
\vspace{-0.15in}
\centering
\small
\setlength{\tabcolsep}{2.5mm}{
  \begin{tabular}{c|cccc}
  % & \multicolumn{4}{c}{\textbf{*** }} \\
   \toprule
   % \vspace{-0.15in}
% &\multicolumn{3}{c}{CIFAR10}\\
   IPC & 1 & 10 & 50\\
   Ratio\%& 0.02 & 0.2 & 1\\
   \midrule
FTD& 46.8$\pm$0.3 & 66.6$\pm$0.3 & 73.8$\pm$0.2 \\
w.ours& 68.7$\pm$0.4 & 73.9$\pm$0.6 & 75.6$\pm$0.3  \\

\bottomrule
     \end{tabular}}
     \vspace{-3mm}
     % \vspace{1em}
  \caption{
Use FTD as baseline method on CIFAR10.}
  \label{tab:ftd}
  \vspace{-0.3in}
\end{table}


==> tables/rebuttal_ratio1.tex <==
\begin{table}[ht!]
\vspace{-0.25in}
\centering
\small
\setlength{\tabcolsep}{2.5mm}{
  \begin{tabular}{cc|cc}
  % & \multicolumn{4}{c}{\textbf{*** }} \\
   \toprule
   % \vspace{-0.15in}
% &\multicolumn{4}{c}{Evaluation Model}\\
   RIPC&Ratio\%&MTT&ours\\
   \midrule
1&0.02& 46.3$\pm$0.8 & \textbf{48.2$\pm$0.9}\\
10&0.2& 65.3$\pm$0.7 & \textbf{66.8$\pm$0.5}\\

\bottomrule
     \end{tabular}}
     \vspace{-3mm}
     % \vspace{1em}
%   \caption{
% Test accuracy using the same number of images and compression ratio on CIFAR10.}
\caption{Use the same number of images and compression ratio on CIFAR10}
  \label{tab:ratio1}
  \vspace{-0.1in}
\end{table}
%在CIFAR10上使用相同的图像数量和压缩率

==> tables/rebuttal_ratio2.tex <==
\begin{table}[ht!]
\vspace{-0.2in}
\centering
\small
\setlength{\tabcolsep}{2.5mm}{
  \begin{tabular}{c|cccc}
  % & \multicolumn{4}{c}{\textbf{*** }} \\
   \toprule
   % \vspace{-0.15in}
% &\multicolumn{4}{c}{Evaluation Model}\\
   RIPC & 10 & 10 & 10 & 10\\
   Ratio\%& 0.2 & 0.1 & 0.05 & 0.02\\
   \midrule
ours& 66.8$\pm$0.5 & 66.3$\pm$0.6 & 65.5$\pm$0.7 & 64.1$\pm$0.3 \\

\bottomrule
     \end{tabular}}
     \vspace{-3mm}
     % \vspace{1em}
  \caption{
Use the same number of images but different compression ratio on CIFAR10.}
  \label{tab:ratio2}
  \vspace{-0.25in}
\end{table}


==> tables/rebuttal_time.tex <==
\begin{table}[ht!]
\vspace{-3mm}
\centering
\small

  \begin{tabular}{c|ccc}
  % & \multicolumn{4}{c}{\textbf{*** }} \\
   \hline
   % \vspace{-0.15in}
    & HaBa & ~\cite{deng2022remember} & ours  \\
   \hline
Time & 25h & 1982.5h & \textbf{8.3h}\\
\hline
     \end{tabular}

 
\vspace{-2mm}
  \caption{Training time of our method with other methods on a single RTX-2080 Ti GPU with CIFAR10, IPC=1.}
\label{tab:rebuttal_t}
\vspace{-7mm}
\end{table}

